ReCraft: Self-Contained Split, Merge, and Membership Change of Raft Protocol

Designing reconfiguration schemes for consensus protocols is challenging because subtle corner cases during reconfiguration could invalidate the correctness of the protocol. Thus, most systems that embed consensus protocols conservatively implement the reconfiguration and refrain from developing an efficient scheme. Existing implementations often stop the entire system during reconfiguration and rely on a centralized coordinator, which can become a single point of failure. We present ReCraft, a novel reconfiguration protocol for Raft, which supports multi- and single-cluster-level reconfigurations. ReCraft does not rely on external coordinators and blocks minimally. ReCraft enables the sharding of Raft clusters with split and merge reconfigurations and adds a membership change scheme that improves Raft. We prove the safety and liveness of ReCraft and demonstrate its efficiency through implementations in etcd.

==> Makefile <==
.PHONY: all embed clean fresh once rtf html docx
LATEX=pdflatex
BIBTEX=bibtex

PAPER=main
BIBFILE=refs.bib
STYFILES=$(wildcard *.sty)
TEXFILES=$(wildcard *.tex)
FIGFILES=$(wildcard ./figs/*.pdf)

all: $(PAPER).pdf

fresh: clean all

once: 
	$(LATEX) $(PAPER)

$(PAPER).pdf: $(TEXFILES) $(BIBFILE) $(FIGFILES) $(STYFILES)
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)

rtf:
	latex2rtf $(PAPER).tex 

html:
	htlatex $(PAPER).tex

docx:
	pandoc -o $(PAPER).docx $(PAPER).tex

# This embeds missing fonts to the pdf
embed: $(PAPER).pdf
	gs  -dPDFSETTINGS=/prepress -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$(PAPER)_embed.pdf -f $(PAPER).pdf
	
#	-c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $(PAPER).pdf

clean:
	rm -f *.aux *.log *~ .DS_Store *.dvi $(PAPER).ps $(PAPER).pdf $(PAPER).rtf\
		*.lot *.lof *.toc *.blg *.bbl *.ent *.bak *.out *.4ct *.4tc *.css \
		*.html *.idv *.lg *.tmp *.xref $(PAPER).docx $(PAPER)_embed.pdf


==> implementation.tex <==
\section{Implementation}
\label{sec:impl}

We implement \sysname{} in etcd version 3.5. We modify the
etcd-Raft~\cite{etcd-raft} library written in Go to implement \sysname{}. 
We modify different parts of etcd to export the new interfaces and
to use the split, merge, and membership change features. It took a total of
4K+ lines of code modifications.

\para{Enabling Wait-Free Reconfigurations.} Etcd does not support applying log
entries in a wait-free fashion for reconfigurations. We add a new special 
reconfiguration log entry type that immediately applies after the log entry is 
appended to the local log. The implementation is not straightforward because 
when the reconfiguration log entry gets overwritten by another log entry, 
the configuration has to revert back to the original configuration. We cache 
the previous configuration for easy revert until the new configuration commits. 

\para{Leader Election after Split.}
After the split, new leaders must be elected in each subcluster. Under a steady 
state, all nodes will receive the message to start the new configuration 
with a little time difference. To avoid waiting for the election timeout, 
we choose one node in each subcluster to start the election immediately after 
applying the new configuration. 

\para{Merge Transaction.}
The first two phases of the merge, or the 2PC logic, are implemented as an 
overlay logic of Raft. The relevant operations execute at the cluster level 
and the internal workings of Raft are barely affected by them until the 
merge transaction commits. Thus, as an implementation, we created a separate 
2PC module that runs with the Raft library and follows the 
2PC-related commands in the log. The module is in every node but activates only
in the leader node. The module retires to finish uncommitted transactions and 
filters duplicate transactions based on the transaction id. 

\para{Snapshot Exchange.} The data exchange and log compaction happen in both 
etcd key-value store and the Raft library layers. We create and exchange the 
snapshots and store the merged snapshot persistently as a file in the etcd 
layer. The Raft layer compacts the SMR log and resets the epoch number. 

\para{Limitations.} Etcd supports atomic transactions over multiple keys by 
committing a bundled transaction log entry. This mechanism works within a 
single shard, but our implementation does not support cross-shard transactions. 
They can be implemented with distributed transactions, such as the 2PC, but we 
leave it as future work. 


%\begin{figure}[h]
%\includegraphics[scale=0.3]{../fig/impl-etcd-parts.png}
%\centering
%\caption[Etcd implementation: 5 main components]
%{Etcd implementation: 5 main components (center)}
%\label{fig:etcd-parts}
%\end{figure}
%
%


==> merge_pseudo_fig.tex <==
\begin{figure*}
%\centering
\scriptsize
\lstdefinelanguage{mypseudo}{ 
	escapeinside={(*}{*)},
	morecomment=[l]{//},
	morecomment=[s]{/*}{*/},
    string=[b]",
	keywords={if, else, foreach, in, return},
    basicstyle={\ttfamily}, % basic font setting
    %morekeywords=[2]{=, ==, !, !=, >, <, ||, &&, &, |},
    %otherkeywords={=, ==, !, !=, >, <, ||, &&, &, |},
	commentstyle=\itshape,
	keywordstyle={\color{blue}},
	keywordstyle=[2]{\color{red}},
    %stringstyle=\color{red},
	%emph={SplitEnterJoint},
    %emphstyle={\bfseries},
}
\lstset{
numbers=left, numberstyle=\tiny, stepnumber=1, numbersep=5pt,
showstringspaces=false, mathescape=true
}
\hspace{0.018\textwidth}
\begin{minipage}[t]{0.31\textwidth}
\begin{lstlisting}[language=mypseudo, firstnumber=1]
// Coordinator cluster leader 
bool (*\textbf{\mergeprepare{}}*)(Config (*\conftx{}*)) {
  $C$ = getCurrentConfig();
  2pcVotes = [];
  votes = [];
  // Precondition check
  if (!P1 || !P2' || !P3) 
    return FAILURE;
  // 2PC prepare for itself
  (*\conftx{}'*) = setDecision((*\conftx{}*), OK);
  foreach (n in memberNodes($C$)) {
    if (appendEntry(n, (*\conftx{}'*)) == OK) 
      votes.add(n); 
  }
  // send 2PC prepare to (*\confsub*)
  foreach ((*\confsub*) in clusters((*\conftx{}*))) { 
    if (2PCPrepare((*\confsub*), (*\conftx{}*)) == OK)
      2pcVotes.add((*\confsub*));   
  (*\conftx{}'*) = setDecision}
  applyConfig((*\conftx{}*)); 
  if (isQuorum($C$, votes) && 
      isUnanimous((*\conftx*), 2pcVotes)) 
    return SUCCESS;
  else return FAILURE;
} 
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\begin{lstlisting}[language=mypseudo, firstnumber=26]
// Non-coordinator cluster leader
bool (*\textbf{\handlemergepreparett{}}*)(Config (*\conftx{}*)) {
  $C$ = getCurrentConfig();
  votes = [];
  // Precondition check
  if (!P1 || !P2' || !P3) res = NO;
  else res = OK;
  (*\conftx{}'*) = setDecision((*\conftx{}*), res);
  foreach (n in memberNodes($C$)) {
    if (appendEntry(n, $C$) == OK) 
      votes.add(n); 
  }
  if (res == OK) applyConfig((*\conftx{}'*));
  if (isQuorum($C$, votes)) {
    respond(res);
    return SUCCESS;
  } 
  else return FAILURE;
}
// Coordinator cluster leader
bool (*\textbf{\mergecommit{}}*)(Config (*\conftx{}, \confnew{}*)) {
  $C$ = getCurrentConfig();
  2pcAcks = [];
  votes = [];
  if (!underTX($C$) || !TXPrepared((*\conftx{}*)))
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\begin{lstlisting}[language=mypseudo, firstnumber=51]
    return FAILURE;
  res = getTXResults((*\conftx{}*));
  $C_{next}$ = (res == COMMIT) ? (*\confnew*) : (*\confabort*);
  foreach (n in memberNodes($C$)) {
    if (appendEntry(n, $C_{next}$) == OK) 
      votes.add(n); 
  }
  // send 2PC prepare to (*\confsub*)
  foreach ((*\confsub*) in clusters((*\conftx{}*))) { 
    if (2PCCommit((*\confsub*), $C_{next}$) == OK)
      2pcAcks.add((*\confsub*));   
  }
  if (isQuorum($C$, votes) &&
      allResponded((*\conftx*), 2pcAcks)) { 
    applyConfig($C_{next}$);
    return SUCCESS;
  else return FAILURE;
}
// Non-coordinator cluster leader
bool (*\textbf{\handlemergecommit{}}*)(Config $C_{next}$) {
  // 1. Regular appendEntry of $C_{next}$      
  //    to all nodes. 
  // 2. Apply $C_{next}$ only after 
  //    confirimg the commit of $C_{next}$. 
}
\end{lstlisting}
\end{minipage}

  \caption{%
	Pseudo code of functions for the merge protocol.
  }%
  \label{fig:mergepseudo}
\end{figure*}

%    if (res == OK) votes.add(n);
%    if (res == PULL) { 
%      pullLog(n); 
%      return FAILURE; 
%  } }
%  if (isQuorum($C$, votes)) 
%    return SUCCESS;
%  else return FAILURE;
%}
%// Follower - response to request vote
%void (*\textbf{\votett{}}*)(Request req) {
%  $E_{curr}$ = getEpoch(getCurrentTerm());
%  $E_{req}$ = getEpoch(req.term);
%  if ($E_{curr}$ > $E_{req}$) respondPull(req.node); 
%  else ...  // same as Raft voting 
%}
%// Follower - response to append entry
%void (*\textbf{\appendtt{}}*)(Request req) {
%	// same as Raft appending
%}
%


==> split_pseudo_fig.tex <==
\begin{figure*}
%\centering
\scriptsize
\lstdefinelanguage{mypseudo}{ 
	escapeinside={(*}{*)},
	morecomment=[l]{//},
	morecomment=[s]{/*}{*/},
    string=[b]",
	keywords={if, else, foreach, in, return},
    basicstyle={\ttfamily}, % basic font setting
    %morekeywords=[2]{=, ==, !, !=, >, <, ||, &&, &, |},
    %otherkeywords={=, ==, !, !=, >, <, ||, &&, &, |},
	commentstyle=\itshape,
	keywordstyle={\color{blue}},
	keywordstyle=[2]{\color{red}},
    %stringstyle=\color{red},
	%emph={SplitEnterJoint},
    %emphstyle={\bfseries},
}
\lstset{
numbers=left, numberstyle=\tiny, stepnumber=1, numbersep=5pt,
showstringspaces=false, mathescape=true
}
\hspace{0.018\textwidth}
\begin{minipage}[t]{0.31\textwidth}
\begin{lstlisting}[language=mypseudo, firstnumber=1]
// Leader - enter joint consensus
bool (*\textbf{\splitenterjointtt{}}*)(Config (*\confjoint{}*)) {
  $C$ = getCurrentConfig();
  votes = [];
  // Precondition check
  if (!P1 || !P2' || !P3) 
    return FAILURE;
  foreach (n in memberNodes($C$)) { 
    if (appendEntry(n, (*\confjoint{}*)) == OK) 
      votes.add(n); 
  }
  applyConfig((*\confjoint{}*)); 
  if (isQuorum($C$, votes)) 
    return SUCCESS;
  else return FAILURE;
} 
// Leader - leave joint consensus
bool (*\textbf{\splitleavejointtt{}}*)(Config (*\confnew{}*)) {
  $C$ = getCurrentConfig();
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\begin{lstlisting}[language=mypseudo, firstnumber=20]
  votes = [];
  if (!isJoint($C$)||!isCommitted($C$)) 
    return FAILURE;
  foreach (n in memberNodes($C$)) {
    if (appendEntry(n, (*\confnew{}*)) == OK) 
      votes.add(n); 
  }
  (*\confsub{}*) = myConfig((*\confnew{}*));
  applyCommitConfig((*\confsub{}*));
  if (isQuorum((*\confsub{}*), votes)) {
    notifyCommit((*\confnew{}*));
    applyElectConfigAndIncEpoch((*\confsub{}*));
    return SUCCESS;
  } 
  else return FAILURE;
}
// Candidate
bool (*\textbf{\requestvotett{}}*)() {
  $C$ = getCurrentConfig();
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\begin{lstlisting}[language=mypseudo, firstnumber=39]
  foreach (n in memberNodes($C$)) { 
    res = requestVote(n)
    if (res == OK) votes.add(n);
    if (res == PULL) { 
      pullLog(n); 
      return FAILURE; 
  } }
  if (isQuorum($C$, votes)) 
    return SUCCESS;
  else return FAILURE;
}
// Follower - response to request vote
void (*\textbf{\votett{}}*)(Request req) {
  $E_{curr}$ = getCurrentEpoch();
  $E_{req}$ = getEpoch(req.term);
  if ($E_{curr}$ > $E_{req}$) respondPull(req.node); 
  else ...  // same as Raft voting 
}


\end{lstlisting}
\end{minipage}

  \caption{%
	Pseudo code of functions for the split protocol.
  }%
  \label{fig:splitpseudo}
\end{figure*}
%// Follower - response to append entry
%void (*\textbf{\appendtt{}}*)(Request req) {
%  // same as Raft appending
%}

